A Survey of Brain Inspired Technologies for Engineering

Cognitive engineering is a multi-disciplinary field and hence it is difficult to find a review article consolidating the leading developments in the field. The in-credible pace at which technology is advancing pushes the boundaries of what is achievable in cognitive engineering. There are also differing approaches to cognitive engineering brought about from the multi-disciplinary nature of the field and the vastness of possible applications. Thus research communities require more frequent reviews to keep up to date with the latest trends. In this paper we shall dis-cuss some of the approaches to cognitive engineering holistically to clarify the reasoning behind the different approaches and to highlight their strengths and weaknesses. We shall then show how developments from seemingly disjointed views could be integrated to achieve the same goal of creating cognitive machines. By reviewing the major contributions in the different fields and showing the potential for a combined approach, this work intends to assist the research community in devising more unified methods and techniques for developing cognitive machines.

==> Pictures/Neuromophic_hardware_tree <==
{"contentType":"application/gliffy+json","version":"1.1","metadata":{"title":"untitled","revision":0,"exportBorder":false},"embeddedResources":{"index":0,"resources":[]},"stage":{"objects":[{"x":615,"y":499,"rotation":0,"id":33,"uid":"com.gliffy.shape.basic.basic_v1.default.text","width":150,"height":27,"lockAspectRatio":false,"lockShape":false,"order":33,"graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 24px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 27px; color: rgb(0, 0, 0);\">Simulation</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null,"linkMap":[]},{"x":235,"y":499,"rotation":0,"id":32,"uid":"com.gliffy.shape.basic.basic_v1.default.text","width":150,"height":27,"lockAspectRatio":false,"lockShape":false,"order":32,"graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 24px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 27px; color: rgb(0, 0, 0);\">Emulation</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null,"linkMap":[]},{"x":140,"y":240,"rotation":0,"id":29,"uid":"com.gliffy.shape.basic.basic_v1.default.round_rectangle","width":340,"height":250,"lockAspectRatio":false,"lockShape":false,"order":23,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.round_rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"none","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[],"linkMap":[]},{"x":690,"y":336,"rotation":0,"id":23,"uid":"com.gliffy.shape.basic.basic_v1.default.line","width":100,"height":100,"lockAspectRatio":false,"lockShape":false,"order":22,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":10,"controlPath":[[5,-1],[5,31.5],[140,31.5],[140,64]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":5,"px":0.5,"py":1}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":15,"px":0.5,"py":0}}},"linkMap":[]},{"x":689,"y":336,"rotation":0,"id":22,"uid":"com.gliffy.shape.basic.basic_v1.default.line","width":100,"height":100,"lockAspectRatio":false,"lockShape":false,"order":21,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":10,"controlPath":[[6,-1],[6,20.730674684008818],[6,42.46134936801769],[6,64.19202405202651]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":5,"px":0.5,"py":1}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":11,"px":0.5,"py":0}}},"linkMap":[]},{"x":692,"y":337,"rotation":0,"id":21,"uid":"com.gliffy.shape.basic.basic_v1.default.line","width":100,"height":100,"lockAspectRatio":false,"lockShape":false,"order":20,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":10,"controlPath":[[3,-2],[3,30.5],[-142,30.5],[-142,63]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":5,"px":0.5,"py":1}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":13,"px":0.5,"py":0}}},"linkMap":[]},{"x":309,"y":335,"rotation":0,"id":20,"uid":"com.gliffy.shape.basic.basic_v1.default.line","width":100,"height":100,"lockAspectRatio":false,"lockShape":false,"order":19,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":10,"controlPath":[[1,0],[1,32.5],[101,32.5],[101,65]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":3,"px":0.5,"py":1}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":9,"px":0.5,"py":0}}},"linkMap":[]},{"x":309,"y":334,"rotation":0,"id":19,"uid":"com.gliffy.shape.basic.basic_v1.default.line","width":100,"height":100,"lockAspectRatio":false,"lockShape":false,"order":18,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":10,"controlPath":[[1,1],[1,33.5],[-99,33.5],[-99,66]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":3,"px":0.5,"py":1}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":7,"px":0.5,"py":0}}},"linkMap":[]},{"x":501,"y":185,"rotation":0,"id":18,"uid":"com.gliffy.shape.basic.basic_v1.default.line","width":100,"height":100,"lockAspectRatio":false,"lockShape":false,"order":17,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":10,"controlPath":[[-16.75,0],[-16.75,37.5],[194,37.5],[194,75]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":0,"px":0.5,"py":1}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":5,"px":0.5,"py":0}}},"linkMap":[]},{"x":503,"y":189,"rotation":0,"id":17,"uid":"com.gliffy.shape.basic.basic_v1.default.line","width":100,"height":100,"lockAspectRatio":false,"lockShape":false,"order":16,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":10,"controlPath":[[-18.75,-4],[-18.75,33.5],[-193,33.5],[-193,71]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":0,"px":0.5,"py":1}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":3,"px":0.5,"py":0}}},"linkMap":[]},{"x":490,"y":240,"rotation":0,"id":31,"uid":"com.gliffy.shape.basic.basic_v1.default.round_rectangle","width":410,"height":250,"lockAspectRatio":false,"lockShape":false,"order":24,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.round_rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"none","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[],"linkMap":[]},{"x":160,"y":400,"rotation":0,"id":7,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":100,"height":75,"lockAspectRatio":false,"lockShape":false,"order":6,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#b6d7a8","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2,"y":0,"rotation":0,"id":8,"uid":null,"width":96,"height":20,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\">Analog</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":360,"y":400,"rotation":0,"id":9,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":100,"height":75,"lockAspectRatio":false,"lockShape":false,"order":8,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#b6d7a8","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2,"y":0,"rotation":0,"id":10,"uid":null,"width":96,"height":20,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\">Digital\n</span></p><p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\"></span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":260,"y":260,"rotation":0,"id":3,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":100,"height":75,"lockAspectRatio":false,"lockShape":false,"order":2,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#6aa84f","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2,"y":0,"rotation":0,"id":4,"uid":null,"width":96,"height":20,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\">Neurochip\n</span></p><p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\"></span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":620,"y":260,"rotation":0,"id":5,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":150,"height":75,"lockAspectRatio":false,"lockShape":false,"order":4,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#6fa8dc","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.999999999999999,"y":0,"rotation":0,"id":6,"uid":null,"width":143.99999999999997,"height":20,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\">Neurocomputing</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":500,"y":400,"rotation":0,"id":13,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":100,"height":75,"lockAspectRatio":false,"lockShape":false,"order":12,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#cfe2f3","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2,"y":0,"rotation":0,"id":14,"uid":null,"width":96,"height":40,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\">Accelerator Boards\n</span></p><p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\"></span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":640,"y":400,"rotation":0,"id":11,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":100,"height":75,"lockAspectRatio":false,"lockShape":false,"order":10,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#cfe2f3","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2,"y":0,"rotation":0,"id":12,"uid":null,"width":96,"height":32,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 14px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 16.5px; color: rgb(0, 0, 0);\">Programmable Gate Arrays</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":780,"y":400,"rotation":0,"id":15,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":100,"height":75,"lockAspectRatio":false,"lockShape":false,"order":14,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#cfe2f3","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2,"y":0,"rotation":0,"id":16,"uid":null,"width":96,"height":40,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\">General Purpose</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":414.25,"y":110,"rotation":0,"id":0,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","width":140,"height":75,"lockAspectRatio":false,"lockShape":false,"order":0,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#e06666","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.8000000000000003,"y":0,"rotation":0,"id":2,"uid":null,"width":134.4,"height":40,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\">Neuromorphic Hardware\n</span></p><p style=\"text-align:center;\"><span style=\"font-size: 18px; font-family: Arial; white-space: pre-wrap; text-decoration: none; line-height: 20.5px; color: rgb(0, 0, 0);\"></span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]}],"background":"#FFFFFF","width":900,"height":526,"maxWidth":5000,"maxHeight":5000,"nodeIndex":38,"autoFit":true,"exportBorder":false,"gridOn":true,"snapToGrid":false,"drawingGuidesOn":true,"pageBreaksOn":false,"printGridOn":false,"printPaper":"LETTER","printShrinkToFit":false,"printPortrait":true,"shapeStyles":{"com.gliffy.shape.basic.basic_v1.default":{"fill":"none","stroke":"#333333","strokeWidth":2,"gradient":false,"shadow":false}},"lineStyles":{"global":{"stroke":"#000000","strokeWidth":2,"orthoMode":1}},"textStyles":{},"themeData":null}}
